Algorithms and tools for iterated Eisenstein integrals

We present algorithms to work with iterated Eisenstein integrals that have recently appeared in the computation of multi-loop Feynman integrals. These algorithms allow one to analytically continue these integrals to all regions of the parameter space, and to obtain fast converging series representations in each region. We illustrate our approach on the examples of hypergeometric functions that evaluate to iterated Eisenstein integrals as well as the well-known sunrise graph.

==> app_coradical.tex <==
% !TEX root = modular_numerics.tex

\section{The coradical filtration}
\label{app:coradical}
We would expect that, whenever an MMV associated to Eisenstein series for $\Gamma(N)$ can be expressed in terms transcendental constants known from MPLs, then these should be MPLs evaluated at the $N$-th root of unity.

This is indeed the case for $\Gamma(2)$. However, when staring at the MMVs for level two, one sees some intriguing patterns:
\begin{itemize}
\item At weight two, we have
\beq
\Lambda(h_{2,1,0}^{(2)};1) = 2\pi\log2\,,\qquad \Lambda(h_{2,0,1}^{(2)};1) = -2\pi\log2\,,\qquad 
\Lambda(h_{2,1,1}^{(2)};1) = 0\,.
\eeq
We see for example that neither $\pi^2$ nor $\log^22$ appears.
\item At weight four and six and length one, we then expect MZVs, powers of $\log2$, $\textrm{Li}_4(1/2)$, etc. to appear. However, we only find MZVs.
\item Powers of $\log2$ and $\textrm{Li}_4(1/2)$ do appear for higher lengths.
\end{itemize}
In the following we explain some of these patterns. Note that his has practical implications: If we know that in some instances some transcendental constants cannot appear, then we can reduce the number of basis elements we need to include in a fit with PSLQ.

\subsection{The coradical filtration}
In Section 2.5 of ref.~\cite{Brown:coaction}, Brown defines a coradical filtration on motivic periods. In the case of MPLs this filtration is easy to describe. In particular, elements of coradical degree 0 are semi-simple elements elements, i.e., algebraic numbers and powers of $2\pi i$. Elements of coradical degree 1 are primitive elements, i.e., here they are MZVs of depth one and odd weight, and logarithms. 

More generally, there is a map $\Phi$ which assigns to a period a tensor product of primitive elements (the `decomposition into primitives' map), multiplied by semi-simple elements. For example
\beq\bsp
\Phi(\zeta_n) &\,= \zeta_n\,,\qquad n\textrm{ odd}\,,\\
\Phi(\log 2) &\,= \log 2\,,\\
\Phi(\textrm{Li}_4(1/2)) &\, = -\frac{7}{8} \zeta_3\otimes \log 2+\frac{\pi ^2}{12}  \log 2\otimes \log2-\log2\otimes \log 2\otimes \log2\otimes \log2\,.
\esp\eeq
The coradical degree is then the `length of the longest tensor'. $\Phi$ is linear with respect to semi-simple elements, and maps product of periods to the shuffle product of the tensors of primitive elements,
\beq
\Phi(a\cdot b) = \Phi(a)\sh\Phi(b)\,.
\eeq
We see for example that $\textrm{Li}_4(1/2)$ has coradical degree four.





==> mmvs.tex <==
% !TEX root = modular_numerics.tex

\section{Special values of iterated integrals of modular forms: Multiple modular values}
\label{sec:mmvs}
The goal of this section is to study certain classes of transcendental constants that appear when iterated integrals of modular forms are evaluated at certain special points. Of particular interest are iterated integrals of modular forms evaluated at rational values of $\tau$ (cf.~eq.~\eqref{eq:example_I}). 
In the remainder of this section we show that in these cases we can express large classes of these integrals in terms of some transcendental number that have recently appeared in the mathematics literature.

For modular forms $h_j$, $1\le j\le k$, of weight $n_j\ge 2$ and integers $m_j$ such that $1\le m_j<n_j$, the associated \emph{multiple modular value} (MMV) is defined by the integral~\cite{Brown:mmv}:
\beq\label{eq:mmv_def}
\Lambda(h_k,\ldots,h_1;m_k,\ldots,m_1) = (-i)^{m}\,\int_0^{i\infty}d\tau_1\,h_1(\tau_1)\,\tau_1^{m_1-1}\int_{0}^{\tau_1}\ldots\int_{0}^{\tau_{k-1}}d\tau_k\,h_k(\tau_k)\,\tau_k^{m_k-1}\,,
\eeq
with $m=m_1+\ldots+m_k$. We note that the restrictions on $m_j$ and $n_j$ that appear in the definition of MMVs are precisely the conditions that define our restricted class of integrals from the previous section.
The integral in eq.~\eqref{eq:mmv_def} may diverge, and we have to interpret it again as a regularised version. We define the weight of an MMV as $n_1+\ldots+n_k$ and the length as $m$. 
MMVs of small weight and lengths associated to modular forms of level one have been studied in ref.~\cite{Brown:mmv,Brown:mmv2}. It is easy to see that MMVs form a shuffle algebra,
\beq\bsp\label{eq:Lambda_def}
\Lambda&(h_l,\ldots,h_{k+1};m_l,\ldots,m_{k+1})\,\Lambda(h_k,\ldots,h_1;m_k,\ldots,m_1) \\
&\,= \sum_{\sigma\in\Sigma(k,l)}\Lambda(h_{\sigma_l},\ldots,h_{\sigma_1};m_{\sigma_k},\ldots,m_{\sigma_1})\,,
\esp\eeq
where the sum runs over all shuffles of $k$ and $l-k$ elements.

In the following we argue that whenever an iterated integral of modular forms (taken from our restricted class) is evaluated at a rational value of $\tau$, then it can be expressed in terms of MMVs. In order to see this, we need to show two things:
\begin{enumerate}
\item We can always bring any integrand into a form that matches the integrands in eq.~\eqref{eq:mmv_def}.
\item Every integration path from $i\infty$ to $r\in\mathbb{Q}$, can be transformed into a sequence of paths $i\infty$ to $0$.
\end{enumerate}

The first point was already discussed in the previous section, so we focus on the second point.
We denote by $\{\alpha,\beta\}=-\{\beta,\alpha\}$, $\alpha,\beta\in\mathbb{Q}\cup\{i\infty\}$ the oriented straight line from $\alpha$ to $\beta$. Path composition is then encoded in the relation
\beq
\{\alpha,\beta\} + \{\beta,\gamma\} = \{\alpha,\gamma\}\,.
\eeq
Since $\SL(2,\mathbb{Z})$ acts on $\mathbb{Q}\cup\{i\infty\}$, we can extend this action to straight line paths via
\beq
\gamma\cdot \{\alpha,\beta\} = \{\gamma\cdot \alpha,\gamma\cdot\beta\}\,,\qquad \gamma\in\SL(2,\mathbb{Z})\,.
\eeq
In ref.~\cite{ManinSymbols} it was that for every straight line path $\{\alpha,\beta\}$, there are $\gamma_1,\ldots,\gamma_r\in\SL(2,\mathbb{Z})$ such that
\beq
\{\alpha,\beta\} = \sum_{p=1}^r \gamma_p\cdot\{0,i\infty\}\,.
\eeq
The matrices $\gamma_i$ can be constructed algorithmically for every path $\{\alpha,\beta\}$ (see, e.g.,~ref.~\cite{steinbook} or Appendix~\ref{app:Manin}). We can use this result to express every iterated integral from our restricted class evaluated at a rational argument in terms of MMVs using the algorithms presented in the previous section. We stress again the importance of working with the restricted class of integrals for this to work. 

Since MMVs are iterated integrals of modular forms, we can apply the method of the previous section and work out what the integrals become under modular transformations. We can use this 

We also note that there is a reflection identity for MMVs associated to Eisenstein series for $\Gamma(N)$,
\beq
\Lambda(h_{N,r_k,s_k}^{(n_k)},\ldots,h_{N,r_1,s_1}^{(n_1)};m_k,\ldots,m_1) = i^n\,\Lambda(h_{N,\tilde{r}_1,\tilde{s}_1}^{(n_1)},\ldots,h_{N,\tilde{r}_k,\tilde{s}_k}^{(n_k)};\tilde{m}_1,\ldots,\tilde{m}_k)\,,
\eeq
where $n$ is the weight of the MMV, and 
\beq
\tilde{m}_j=n_j-m_j\,,\qquad \tilde{r}_j = N-s_j\,,\qquad \tilde{s}_j = r_j\,.
\eeq
The reflection identity can easily be obtained by working out the transformation of the corresponding iterated integrals under the modular transformation $S:\tau\to -1/\tau$.
MMVs are (conjecturally transcendental) constants. In applications it is important to obtain their numerical value. Since MMVs are special cases of iterated integrals of modular forms, namely those evaluated at $\tau=0$, we can try to proceed in the same way as for iterated integrals and evaluate them numerically using $q$-expansions. In this case, however, the expansion parameter is $q_N=1$, which leads to badly converging expansions. In the next section we describe a way to accelerate the convergence of the series.








==> setup_2F1.tex <==
% !TEX root = modular_numerics.tex

\section{An invitation}
\label{sec:invitation}
The aim of this section is to illustrate the content and the goal of this paper on a simple example, namely the family of elliptic hypergeometric ${}_2F_1$ functions defined by
\begin{align}\label{eq:2F1_def}
T(n_1,n_2,n_3;z) = \int_0^1 dx\, x^{-1/2 + n_1 + a\, \epsilon} (1-x)^{-1/2 + n_2 + b \epsilon} (1-z\, x)^{-1/2 + n_3 + c\,\epsilon}\,.
\end{align}
where $n_i\in\mathbb{Z}$ and $a,b,c$ are complex numbers. The integral defines a meromorphic function of $\eps$, and we interpret the integral as a Laurent series in $\eps$. In the following we assume that $z$ is real. As long as $z<1$ the integral is real order by order in $\eps$, but it develops an imaginary part when $z>1$. We assume that the branches of all functions are determined by assigning a small positive imaginary part to $z$.

It is easy to show that all integrals in the family in eq.~\eqref{eq:2F1_def} can be expressed as a linear combination of two independent master integrals, which can be chosen as
\begin{equation}
T_1(z) = T(0,0,0;z)\,, \quad T_2(z) = T(1,0,0;z)\,.
\end{equation} 
The master integrals were evaluated order-by-order in ref.~\cite{Broedel:2017kkb,Broedel:2018iwv,Broedel:2018rwm} in terms of elliptic polylogarithms and iterated integrals of Eisenstein series for the congruence subgroup $\Gamma(2) = \{\gamma\in\SL(2,\mathbb{Z}):\gamma=1\!\!\mod 2\}$. Iterated integrals of Eisenstein series are a special case of iterated integrals of modular forms defined by~\cite{ManinModular,Brown:mmv}
\beq\label{eq:IEI_def}
I(h_1,\ldots,h_k;\tau) = \int_{i\infty}^{\tau}d\tau'\,h_1(\tau')\,I(h_2,\ldots,h_k;\tau')\,,\quad I(;\tau)=1\,,
\eeq
where $h_i$ are modular forms of weight $n_i$ for a certain subgroup $\Gamma\subseteq \SL(2,\mathbb{Z})$. A detailed discussion of modular forms will be given in Section~\ref{sec:modular_forms}. For now, it suffices to say that each $h_i$ is a holomorphic function from the extended upper half plane $\overline{\mathbb{H}} = \mathbb{H}\cup\{i\infty\}\cup\mathbb{Q}$ into the complex numbers such that, if $\left(\begin{smallmatrix}a & b\\ c& d\end{smallmatrix}\right)\in\Gamma$, then
\beq\label{eq:modular_form_trafo}
h_i\left(\frac{a\tau+b}{c\tau+d}\right) = (c\tau+d)^{n_i}\,h_i(\tau)\,.
\eeq
The variable $\tau$ in eq.~\eqref{eq:IEI_def} is related to the variable $z$ in eq.~\eqref{eq:2F1_def} via
\beq
\tau = \frac{\cK_2(z)}{\cK_1(z)} = i\,\frac{\K(1-z-i0)}{\K(z+i0)}\,,
\eeq
where $\K(z)$ denotes the complete elliptic integral of the first kind,
\beq
\K(z) = \int_0^1\frac{dx}{\sqrt{(1-x^2)(1-zx^2)}}\,.
\eeq
We deliberately distinguish here between the functions $\cK_1(z)$ and $\cK_2(z)$ and the complete elliptic integral $\K(z)$: the functions $\cK_1(z)$ and $\cK_2(z)$ span the solution space of a second-order differential operator, and are well defined for all (real) values of $z$. They can always be expressed in terms of elliptic integrals of the first kind, though careful analytic continuation is needed. For $0<z<1$, $\cK_1(z)$ is real and $\cK_2(z)$ is pure imaginary. We can analytically continue  $\cK_1(z)$ and $\cK_2(z)$ to the whole real line using the formula,
\beq
K(z+i0) = \frac{1}{\sqrt{z}}\,\left[\K(1/z) + i\,\K(1-1/z)\right]\,,\quad z>1\,.
\eeq
We then need to split the real axis into three regions:
\begin{enumerate}
\item Region I: $z<0$,
\beq
\cK_1(z) = 2\,\K(z)\,,\qquad \cK_2(z) = \frac{2i}{\sqrt{1-z}}\,\left[\K\left(\frac{1}{1-z}\right) - i\,\K\left(\frac{z}{z-1}\right)\right]\,.
\eeq
\item Region II: $0<z<1$,
\beq
\cK_1(z) = 2\,\K(z)\,,\qquad \cK_2(z) = 2i\,\K(1-z)\,.
\eeq
\item Region II: $z>1$,
\beq
\cK_1(z) = \frac{2}{\sqrt{z}}\,\left[\K\left(\frac{1}{z}\right) + i\,\K\left(1-\frac{1}{z}\right)\right]\,,\qquad \cK_2(z) = 2i\,\K(1-z)\,.
\eeq
\end{enumerate}

Using the explicit expressions for $\cK_1(z)$ and $\cK_2(z)$ in terms of elliptic integrals, we can see that in Region II $\tau$ is purely imaginary. In this region all iterated integrals of modular forms admit a (fast-converging) $q$-expansion, i.e., and expansion of the form
\beq\label{eq:IEI_to_q}
I(h_1,\ldots,h_k;\tau) = \sum_{p=0}^k\sum_{n=0}^{\infty}a_{p,n}\,q_2^n\,\log^pq_2\,,\qquad q_N = e^{2\pi i\tau/N}\,.
\eeq
If $\tau$ is purely imaginary, then $0<q_N<1$, and the series is converging (fast). In Region I \& III, however, $\tau$ develops a non-zero real part. It is easy to check that we have,
\beq\label{eq:tau_i_def}
\tau=\left\{\begin{array}{ll}
1+\tau_1\,, & z<0\,,\\
\tau_2\,, & 0<z<1\,,\\
{\tau_3}/({\tau_3-1})\,,& z>1\,,
\end{array}\right.
\eeq
where the $\tau_i$ are purely imaginary.
Hence, if we can find transformation formul\ae\ for to express $I\!\left(h_1,\ldots,h_k;\frac{a\tau_i+b}{c\tau_i+d}\right)$ in terms of $I(h_1,\ldots,h_k;\tau_i)$, we can obtain fast-converging $q$-expansions in each of the three regions. The strategy for deriving such transformation formul\ae\ is clear: we start from the integral representation in eq.~\eqref{eq:IEI_def} and change variables according to
$\tau'\to \frac{a\tau'+b}{c\tau'+d}$, and then integrate back to obtain iterated integrals evaluated in $\tau_i$. 

While the general strategy is clear, there are several hurdles when trying to implement this strategy in practise:
\begin{enumerate}
\item After the change of variables, the modular forms $h_i$ in the integrand change according to
\beq
d\tau'\,h_i(\tau') \to \frac{d\tau'}{(c\tau'+d)^2}\,h_i\left(\frac{a\tau+b}{c\tau+d}\right)\,.
\eeq
We would then like to apply eq.~\eqref{eq:modular_form_trafo} to obtain a genuine modular form in the integrand. However, it is easy to check that the transformations in eq.~\eqref{eq:tau_i_def} are not in $\Gamma(2)$, and so eq.~\eqref{eq:modular_form_trafo} does not apply. We therefore need to understand how modular forms for $\Gamma$ transform under modular transformations that are not in $\Gamma$. 
%
\item The change of variables also affects the boundaries of integration. In particular, the lower boundary changes from $i\infty$ to $a/c\in\mathbb{Q}\cup\{i\infty\}$. We can use the path composition and path reversal formul\ae\ for iterated integrals to rewrite the integral as a combination of integrals where the lower integration boundary is infinite,
\beq
I(h_1,\ldots,h_k;\tau) = \sum_{p=0}^k (-1)^{k-p}\,I(h_1,\ldots,h_p;\tau) \,I(h_{k},\ldots,h_{p+1};a/c) \,.
\eeq
In this way we introduce transcendental constants corresponding to iterated integrals of modular forms evaluated at rational numbers. We therefore need to understand these numbers, e.g., how to obtain their numerical value or what is there relationship to other kinds of transcendental constants that appear in multi-loop computations. 
%
\item The integrals in eq.~\eqref{eq:IEI_def} may have a logarithmic end-point singularity at $\tau=i\infty$, and only make sense as suitably regularised versions~\cite{Brown:mmv}. The effect of the regularisation is the appearance of logarithms in eq.~\eqref{eq:IEI_to_q}. These logarithms lead to subtleties when performing the change of variables, as we explain on an example. Consider the ordinary Eisenstein series of level 1,
\beq
G_{2k}(\tau) = \sum_{\substack{(m,n)\in\mathbb{Z}^2\\ (m,n)\neq (0,0)}}\frac{1}{(m\tau+n)^{2k}}\,.
\eeq
For $k=2$, its integral admits the $q$-expansion
\beq\label{eq:I_G4_q}
I(G_4;\tau) = -\frac{i\pi^3}{90}\,\log q_1 + i\pi^3\sum_{n=1}^\infty a_n\,q_1^n 
= \frac{\pi^4}{45}\,\tau + i\pi^3\sum_{n=1}^\infty a_n\,q_1^n\,,\qquad a_n\in\mathbb{Q}\,.
\eeq
Next, write $\tau=1+\tau_1$. We have
\beq
I(G_4;1+\tau_1) = \int_{i\infty}^{1+\tau_1}d\tau'\,G_4(\tau')\,.
\eeq
We can change variables $\tau'\to 1+\tau'$. The integrand is invariant under this change of variables, because $G_4(1+\tau') = G_4(\tau')$. Since, naively, the lower integration boundary does not change under translations, we are led to believe that $I(G_4;1+\tau_1)$ is identical to $I(G_4;\tau_1)$. It is easy to see from eq.~\eqref{eq:I_G4_q} to see that this cannot be correct: since $e^{2\pi i(\tau_1+1)}=e^{2\pi i\tau_1} = q_1$, we see that the power series part in eq.~\eqref{eq:I_G4_q} remains unchanged. The first term, however, does change, and we find,
\beq
I(G_4;1+\tau_1) = I(G_4;\tau_1) + \frac{\pi^4}{45}\,.
\eeq
We see that, due to the regularisation and the logarithmic terms in the $q$-expansion, care is needed when performing change of variables.
\end{enumerate}

In the remainder of this paper we present an algorithm to deal with the aforementioned issues.

